Extension of gyrokinetics to transport time scales

Gyrokinetic simulations have greatly improved our theoretical understanding of turbulent transport in fusion devices. Most gyrokinetic models in use are delta-f simulations in which the slowly varying radial profiles of density and temperature are assumed to be constant for turbulence saturation times, and only the turbulent electromagnetic fluctuations are calculated. New massive simulations are being built to self-consistently determine the radial profiles of density and temperature. However, these new codes have failed to realize that modern gyrokinetic formulations, composed of a gyrokinetic Fokker-Planck equation and a gyrokinetic quasineutrality equation, are only valid for delta-f simulations that do not reach the longer transport time scales necessary to evolve radial profiles. In tokamaks, due to axisymmetry, the evolution of the axisymmetric radial electric field is a challenging problem requiring substantial modifications to gyrokinetic treatments. In this thesis, I study the effect of turbulence on the global electric field and plasma flows. By studying the current conservation equation, or vorticity equation, I prove that the long wavelength, axisymmetric flow must remain neoclassical and I show that the tokamak is intrinsically ambipolar, i.e., the radial current is zero to a very high order for any long wavelength radial electric field. Intrinsic ambipolarity is the origin of the problems with the modern gyrokinetic approach since the lower order gyrokinetic quasineutrality (if properly evaluated) is effectively independent of the radial electric field. I propose a new gyrokinetic formalism to solve for the global radial electric field.

==> app_GKeq_delta2.tex <==
\chapter{Gyrokinetic equation in physical phase space to second
order} \label{app_GKeq_delta2}


\begin{equation}
f_i (\bR, E, \mu, t) \simeq f_{ig} + E_1 \frac{\partial
f_{ig}}{\partial E_0} + \mu_1 \frac{\partial f_{ig}}{\partial
\mu_0},
\end{equation}

\noindent with $f_{ig} \equiv f_i (\bR_g, E_0, \mu_0, t)$. Here,
$f_i = f_{Mi} + h_{i1} + h_{i2}$, and in the higher order terms
$(Ze\phiwig/M) (\partial f_{ig}/\partial E_0)$ and $\mu_1
(\partial f_{ig}/\partial \mu_0)$, only $f_{Mi}$ and the
neoclassical piece $h_{i1}^\mathrm{nc}$, which leads to
\begin{equation}
f_i (\bR, E, \mu, t) \simeq f_{ig} + E_1 \frac{\partial}{\partial
E_0} (f_{Mi} + h_{i1}^\mathrm{nc}) + \mu_1 \frac{\partial
h_{i1}^\mathrm{nc}}{\partial \mu_0},
\end{equation}

\noindent Similarly,
\begin{equation}
\frac{\partial f_i}{\partial t} = \frac{\partial f_{ig}}{\partial
t} + E_1 \frac{\partial}{\partial t} \left [
\frac{\partial}{\partial E_0} (f_{Mi} + h_{i1}^\mathrm{nc}) \right
] + \mu_1 \frac{\partial^2 h_{i1}^\mathrm{nc}}{\partial t \partial
\mu_0},
\end{equation}
\begin{equation}
\nabla_\bR f_i = \nabla_{\bR_g} f_{ig} + E_1 \nabla_{\bR_g} \left
[ \frac{\partial}{\partial E_0} (f_{Mi} + h_{i1}^\mathrm{nc})
\right ] + \mu_1 \nabla_{\bR_g} \left ( \frac{\partial
h_{i1}^\mathrm{nc}}{\partial \mu_0} \right )
\end{equation}

\noindent and
\begin{equation}
\frac{\partial f_i}{\partial E} = \frac{\partial f_{ig}}{\partial
E_0} + E_1 \frac{\partial^2}{\partial E_0^2}(f_{Mi} +
h_{i1}^\mathrm{nc}) + \mu_1 \frac{\partial^2
h_{i1}^\mathrm{nc}}{\partial E_0 \partial \mu_0} \right )
\end{equation}

\noindent With these values, the gyrokinetic Fokker-Planck
equation \eq{FP_final} becomes
\begin{equation}
\frac{\partial f_{ig}}{\partial t} + [ u \bun(\bR) + \bv_d ] \cdot
\nabla_{\bR_g} \br \cdot \left ( \nablaave f_{ig} - \frac{Ze}{M}
\nablaave \phiave \frac{\partial f_{ig}}{\partial E_0} \right ) +
E_1 \left [ u \bun(\bR) \cdot \nabla_{\bR_g} \left (
\frac{\partial h_{i1}^\mathrm{nc}}{\partial E_0} \right ) + \bv_M
\cdot \nabla_{\bR_g} \left (\frac{\partial f_{Mi}}{\partial E_0}
\right ) \right ] + \mu_1 \left [ u \bun(\bR) \cdot \nabla_{\bR_g}
\left ( \frac{\partial h_{i1}^\mathrm{nc}}{\partial \mu_0} \right
) + \bv_M \cdot \nabla_{\bR_g} \left (\frac{\partial
f_{Mi}}{\partial \mu_0} \right ) \right ] = \langle C \{ f_i \}
\rangle, \label{FP_delta2_phys_1}
\end{equation}

\noindent where I have used that in statistical equilibrium,
$\partial f_{Mi}/\partial t = 0 = \partial h_{i1}^\mathrm{nc} /
\partial t$. To simplify this equation, it is useful to employ
\begin{eqnarray}
E_1 \left [ u \bun(\bR) \cdot \nabla_{\bR_g} \left (
\frac{\partial h_{i1}^\mathrm{nc}}{\partial E_0} \right ) + \bv_M
\cdot \nabla_{\bR_g} \left (\frac{\partial f_{Mi}}{\partial E_0}
\right ) \right ] = E_1 \frac{\partial}{\partial E_0} \left [ u
\bun(\bR) \cdot \nabla_{\bR_g} \partial h_{i1}^\mathrm{nc} + \bv_M
\cdot \nabla_{\bR_g} \partial f_{Mi} \right ] - E_1 \frac{\partial
v_{||}}{\partial E_0} \bun \cdot \nabla_{\bR_g} h_{i1}^\mathrm{nc}
- E_1 \frac{\partial \bv_M}{\partial E_0} \cdot \nabla_{\bR_g}
f_{Mi}
\end{eqnarray}

\noindent and
\begin{eqnarray}
\mu_1 \left [ u \bun(\bR) \cdot \nabla_{\bR_g} \left (
\frac{\partial h_{i1}^\mathrm{nc}}{\partial \mu_0} \right ) +
\bv_M \cdot \nabla_{\bR_g} \left (\frac{\partial f_{Mi}}{\partial
\mu_0} \right ) \right ] = \mu_1 \frac{\partial}{\partial \mu_0}
\left [ u \bun(\bR) \cdot \nabla_{\bR_g} \partial
h_{i1}^\mathrm{nc} + \bv_M \cdot \nabla_{\bR_g} \partial f_{Mi}
\right ] - \mu_1 \frac{\partial v_{||}}{\partial \mu_0} \bun \cdot
\nabla_{\bR_g} h_{i1}^\mathrm{nc} - \mu_1 \frac{\partial
\bv_M}{\partial \mu_0} \cdot \nabla_{\bR_g} f_{Mi}.
\end{eqnarray}

\noindent Then, equation \eq{FP_delta2_phys_1} reduces to
\begin{equation}
\frac{\partial f_{ig}}{\partial t} + [ u \bun(\bR) + \bv_d ] \cdot
\nabla_{\bR_g} \br \cdot \left ( \nablaave f_{ig} - \frac{Ze}{M}
\nablaave \phiave \frac{\partial f_{ig}}{\partial E_0} \right ) +
E_1 \left [ u \bun(\bR) \cdot \nabla_{\bR_g} \left (
\frac{\partial h_{i1}^\mathrm{nc}}{\partial E_0} \right ) + \bv_M
\cdot \nabla_{\bR_g} \left (\frac{\partial f_{Mi}}{\partial E_0}
\right ) \right ] + \mu_1 \left [ u \bun(\bR) \cdot \nabla_{\bR_g}
\left ( \frac{\partial h_{i1}^\mathrm{nc}}{\partial \mu_0} \right
) + \bv_M \cdot \nabla_{\bR_g} \left (\frac{\partial
f_{Mi}}{\partial \mu_0} \right ) \right ] = \langle C \{ f_i \}
\rangle - E_1 \frac{\partial}{\partial E_0} C^{(\ell)} \{
h_{i1}^\mathrm{nc} \} - \mu_1 \frac{\partial}{\partial \mu_0}
C^{(\ell)} \{ h_{i1}^\mathrm{nc} \}, \label{FP_delta2_phys_1}
\end{equation}


==> app_deltaf.tex <==
\chapter{Turbulent transport of angular momentum in up-down
symmetric tokamaks}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Flux tube $\delta f$ model}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In a flux tube formulation, only the short wavelength components
of $h_i$ and $\phi$ are solved for, where $f_i = f_{Mi} (\psi_R,
E) + h_i (\bR, E, \mu, \sigma, t)$, $\sigma = v_{||}/|v_{||}|$ and
$\psi_R = \psi + \Omega_i^{-1} (\bv \times \bun) \cdot \nabla
\psi$. The $\delta f$ equation \eq{deltaf_FP} is written in terms
of the function $H = h_i + (Ze\phiave/T_i) f_{Mi}$, giving
\begin{equation}
\frac{\partial H}{\partial t} + [u \bun(\bR) + \bv_M] \cdot
\nabla_\bR H - \frac{c}{B} (\nabla_\bR \phiave \times \bun) \cdot
\nabla_\bR H = \frac{Ze}{T_i} f_{Mi} \left ( \frac{\partial
\phiave}{\partial t} + i \omega_\ast^{n, T} \phiave \right ).
\label{deltaf_GK_1}
\end{equation}

\noindent The frequency $\omega_\ast^{n,T}$ is given in
\eq{general_omegastar}. The nonlinear term $(\nabla_\bR \phiave
\times \bun) \cdot \nabla_\bR H$ is singled out in
\eq{deltaf_GK_1}. Given $H$, the quasineutrality gyrokinetic
equation can be written from \eq{qn_mod} to give
\begin{equation}
n_{e1} + n_{e0} \frac{Ze\phi}{T_i} - \int d^3v\, H (\bR_g, E_0,
\mu_0, \sigma, t) = 0, \label{deltaf_qn_1}
\end{equation}

\noindent where the terms $n_{ip} \{\phi\}$ and $\int d^3v\,
(Ze\phiave/T_i) f_{Mi}$ combined to give the adiabatic term
$(e\phi/T_i) n_{e0}$. Here the electron density is divided into a
background density $n_{e0} (\psi)$ and a turbulent piece $n_{e1}$.
To simplify the derivation, I will assume that the electrons are
adiabatic, i.e.,
\begin{equation}
n_{e1] = n_{e0} \frac{e}{T_e} ( \phi - \langle \phi \rangle_\psi
), \label{electron_adiabatic}
\end{equation}

\noindent where the flux surface averaged piece $\langle \phi
\rangle_\psi$ is extracted because the electrons cannot move from
one flux surface to the next.

Equations \eq{deltaf_GK_1} and \eq{deltaf_qn_1} are the most
common gyrokinetic $\delta f$ formulation. 

\begin{equation}
H_i = \sum_{k_\alpha, k_\psi} H_{k_\alpha, k_\psi} (\theta) \exp (
i k_\alpha \alpha_R + i k_\psi \psi_R ),
\end{equation}

\noindent with $\alpha = \zeta - q(\psi) \theta$, $\alpha_R =
\alpha + \Omega_i^{-1} (\bv \times \bun) \cdot \nabla \alpha$ and
$\psi_R = \psi + \Omega_i^{-1} (\bv \times \bun) \cdot \nabla
\psi$. The potential is given in a similar form. Equation
\eq{deltaf_FP} becomes
\begin{eqnarray}
\frac{\partial H_{k_\alpha, k_\psi}}{\partial t} + v_{||} \bun
\cdot \nabla \theta \frac{\partial H_{k_\alpha, k_\psi}}{\partial
\theta} + i \left [ k_\alpha \bv_M \cdot \nabla \alpha + (k_\psi +
k_\alpha q s \theta) \bv_M \cdot \nabla \psi \right ] H_{k_\alpha,
k_\psi} \nonumber \\ - \langle C^{(\ell)} \{ H_{k_\alpha, k_\psi}
\} \rangle + c \sum_{k_\alpha^\prime, k_\psi^\prime} J_0(z^\prime)
( k_\alpha k_\psi^\prime - k_\psi k_\alpha^\prime )
\phi_{k_\alpha^\prime, k_\psi^\prime} H_{k_\alpha -
k_\alpha^\prime, k_\psi - k_\psi^\prime} = \nonumber \\
\frac{Ze}{T_i} J_0 (z) \left ( \frac{ \partial \phi_{k_\alpha,
k_\psi}}{\partial t} + i \omega_\ast^{n,T} \phi_{k_\alpha, k_\psi}
\right ), \label{fluxtube_FP}
\end{eqnarray}

\noindent with $J_0 (z)$ the Bessel function of the first kind, $z
= k_\bot v_\bot/\Omega_i$, $z^\prime = k_\bot^\prime
v_\bot/\Omega_i$ and $k_\bot^2 = k_\alpha^2 |\nabla \alpha|^2 +
k_\psi^2 | \nabla \psi |^2$. The gyrokinetic quasineutrality
equation becomes
\begin{equation}
[1 - \Gamma_0 (b)] \phi_{k_\alpha, k_\psi} = \frac{e n_{e0}}{T_e}
( \phi - \langle \phi \rangle_\psi ) - \frac{en_{e0}}{T_i} \phi -
\int d^3v\, J_0(z) H, \label{fluxtube_qn}
\end{equation}

\noindent with $\Gamma_0 (b) = I_0 (b) \exp ( -b )$, $I_0(b)$ the
modified Bessel function of the first kind and $b = k_\bot^2 M c^2
T_i/Z^2 e^2 B^2$. If in both equation \eq{fluxtube_FP} and
\eq{fluxtube_qn} I change $\theta \rightarrow - \theta$, $v_{||}
\rightarrow - v_{||}$, $k_\psi \rightarrow - k_\psi$, $\phi
\rightarrow - \phi$ and $H \rightarrow - H$, the equations remain
the same. That means that is always possible to find a solution
such that
\begin{equation}
\phi_{k_\alpha, k_\psi} (\theta, t) = - \phi_{k_\alpha, - k_\psi}
(-\theta, t)
\end{equation}

\noindent and
\begin{equation}
H_{k_\alpha, k_\psi} (\theta, E, \mu, \sigma, t) = - H_{k_\alpha,
- k_\psi} (-\theta, E, \mu, \sigma, t),
\end{equation}

\noindent with $\sigma = v_{||}/|v_{||}|$. Then, the flux surface
averaged Reynolds stress
\begin{eqnarray}
\langle R \zun \cdot \matrixtop{\pibf}_i \cdot \nabla \psi
\rangle_\psi = - \frac{1}{V^\prime} \int \frac{d\theta}{\bB \cdot
\nabla \theta} \frac{cI}{B} \sum_{k_\alpha, k_\psi} k_\alpha
\phi_{k_\alpha, k_\psi} \int d^3v\, J_0 (z) H_{-k_\alpha, -k_\psi}
v_{||} \nonumber \\ - \frac{1}{V^\prime} \int \frac{d\theta}{\bB
\cdot \nabla \theta} \frac{c}{B\Omega_i} \sum_{k_\alpha, k_\psi}
k_\alpha k_\psi \phi_{k_\alpha, k_\psi} \int d^3v\, \frac{J_1
(z)}{z} H_{-k_\alpha, -k_\psi} v_\bot^2.
\end{eqnarray}

